Sequential Learning Of Neural Networks for Prequential MDL

Minimum Description Length (MDL) provides a framework and an objective for principled model evaluation. It formalizes Occam's Razor and can be applied to data from non-stationary sources. In the prequential formulation of MDL, the objective is to minimize the cumulative next-step log-loss when sequentially going through the data and using previous observations for parameter estimation. It thus closely resembles a continual- or online-learning problem. In this study, we evaluate approaches for computing prequential description lengths for image classification datasets with neural networks. Considering the computational cost, we find that online-learning with rehearsal has favorable performance compared to the previously widely used block-wise estimation. We propose forward-calibration to better align the models predictions with the empirical observations and introduce replay-streams, a minibatch incremental training technique to efficiently implement approximate random replay while avoiding large in-memory replay buffers. As a result, we present description lengths for a suite of image classification datasets that improve upon previously reported results by large margins.

==> 0X-mdl.tex <==
\section*{\centering Sequential Learning of Neural Networks for Prequential MDL \\ Supplementary Material}\label{sec:App}

\section{The Minimum Description Length Principle}

In this section we try to give a short overview of the mathematical formulation of the Minimum Description Length Principle (MDL). 
For a proper introduction we refer to \citep{Rissanen1984} and \citep{Grunwald2004-fm}.

Like other closely related approaches such as Minimum Message Length~\citep{Wallace2005}, 
MDL is based on the fundamental idea that learning and comprehension correspond to compression 
\citep{Hutter:11uiphil}: Given data $\DD{=}\{y_t\}_i^T$ and a hypothesis space $\mathcal{M} = \{M_1, M_2, \dots \}$, each referring to a probabilistic model $p(\DD | \prm, M_i)$ , the most plausible model 
$M \in \MM$ is the one that yields the shortest description of the data, i.e. compresses it the most. To simplify the notation in this section we will use $\DD{=}\{y_t\}_i^T$ to denote the predicted data only and omit the explicit conditioning on $x_t$.
We use code and model interchangeably, since according to Kraft–McMillan's inequality, the negative logarithm of probability mass functions corresponds to code-length functions.

A crude way to obtain a description length is to consider $L(\DD\,|\,M){=}L_M(\prm){+}L_M(\DD\,|\, \prm)$, where 
$L_M(\prm)$ is the cost of encoding the parameters and $L_M(\DD|\prm)=-\log p(\DD|\prm, M)$ 
is the cost of compressing the data with the parameterized model.
While this approach might be intuitive, it is suboptimal and does not specify how to encode the parameters.
To avoid the ambiguity that comes with choosing a code $L_M(\prm)$ for the parameters, 
the MDL literature instead suggests to use a \emph{universal code} $\overline p(\DD\,|\,M)$, which is 
defined to be the distribution that as closely as possible tracks the code-length of the maximum 
log-likelihood solution within $M$ on all possible data $z_{1:T} \in \YY^T$:
%
\begin{align}
\overline p(\cdot\,|\,M) := 
  \argmin_{q} \max_{z_{1:T} \in \YY^T}
  \left({-}\log q(z_{1:T})- \big({-}\log p(z_{1:T}\,|\,\prmmle(z_{1:T}), M) \big)\right).
\label{eq:universal-dist}
\end{align}

If it exists, the solution of $q$ in \eqref{eq:universal-dist} is the Normalized Maximum Likelihood (NML) 
$p_\text{NML}(y_{1:n}|M) = \sfrac{p(y_{1:n}|\prmmle(y_{1:n}), M)}{\sum_{z_{1:T} \in \YY^n} p(z_{1:T}|\prmmle(z_{1:T}), M)}$. 
Hence, the NML code-length is

\begin{align}
L_\text{NML}(y_{1:T}\,|\,M )= 
    - \underbrace{\vphantom{\log\sum_{z_{1:T} \in \mathcal Y^T} p(z_{1:T}\,|\,\prmmle(z_{1:T}), M)}\log p(\DD\,|\,\prmmle(\DD), M)}_{\text{Log-likelihood of data}}
    + \underbrace{\log\sum_{z_{1:T} \in \mathcal Y^n} p(z_{1:T}|\prmmle(z_{1:T}), M)}_{\text{Model complexity}}
\label{eq:nml-code}
\end{align}

\eqref{eq:nml-code} has two terms: the log-likelihood term, assessing how well the model fits the data, and the model complexity term, formalising Occam's Razor. Intuitively, a model's complexity is large if it can fit well many possible sequences. As a result, using the universal code for model selection leads to favoring models that have expressiveness to model the observed data $\DD$, but do not waste expressiveness on dissimilar data.

Comparing to ERM, MDL doesn't need to have separate validation data, which means the entirety of the dataset can be used for training purpose. In addition, MDL applies for i.i.d data as well as non-stationarity data. 


\subsection{Practical interpretations of MDL}
Although NML is intuitive to understand, it is intractable and even undefined in many cases. There are two other versions of MDL which are also provably universal codes and, in addition, easier to compute in practice:

\paragraph{Bayesian and variational two-part codes.}
In the Bayesian approach, we choose a prior $p(\theta\,|\,M)$ over the parameters. The Bayesian interpretation of the MDL results in a code-length $L_{Bayes}(\DD)=-\log \int_{\theta} p(\DD\,|\,\prm)p(\prm) d\prm$. One can show that the Bayesian code is a universal code \citep{Hutter:03optisp} and it is equivalent to Bayesian model selection with marginal-likelihood. The variational approximation to the Bayesian posterior can be considered a two part-code and makes it feasible to obtain an upper bound on the 
Bayesian description length. 
By sampling the parameters from an approximation $q(\theta)$ to the posterior distribution $p(\theta\,|\,\DD, M)$, the code-length is equivalent to the negated ELBO objective in variational inference:
$$
L_{var}(\DD\,|\,M) = KL[q(\prm)\,||\,p(\prm\,|\,M)] - \E{\prm \sim q}{\log p(\DD\,|\,\prm, M)}
$$

\paragraph{Prequential code.}

We can think of prequential coding as forward validation, where the loss incurs when predicting the datapoint $y_{t+1}$ based on previously datapoints $y_{1:t}$.
The code-length $L_{preq}(\DD\,|\,M)=-\sum_{t=1}^T{\log p(y_t|\hat{\theta}(y_{<t}), M)}$, where $\hat{\prm}(y_{<t})$ is an estimator of the parameters after seeing $t-1$ datapoints.
Typically, $\hat{\prm}(\cdot)$ is a regularized maximum likelihood estimator, but for many reasonable choices of $\hat{\prm}(\cdot)$, the resulting prequential (plug-in) code is a 
universal model despite not having an explicit model complexity term.

In practice, the prequential code can be shorter than that of the approximated Baysian code, especially for neural networks \citep{Blier2018-rl}. 
Unlike Bayesian MDL which requires a Bayesian neural network, prequential MDL can work with any model architecture and optimizer.
A central property that makes the prequential approach attractive for Neural Networks is that any prediction system that predicts the next-step log-loss given the previous data leads to a valid description length. There are no constraints on the type or implementation of the system as long as it obeys the sequential nature of the data and is deterministic (given the PRNG seeds). 
Even a naive system that predicts a uniform distribution over all outcomes constitutes a valid system. 
It leads to a description length of $T \log(\text{number-of-classes})$ and can be considered an upper bound for all sensible systems.

However, the choice and properties of the prequential estimator are important when considering the optimality of the code-length. 
Regularized maximum likelihood estimators for the next-step plug-in distribution generally lead to code-lengths that can be considered optimal for that model family because they form a universal-code \citep{rissanen1987stochastic}. 
If it exists, it coincides with the normalized maximum-likelihood code-length up to neglectable offsets
\citep{rissanen1987stochastic, grunwald2007minimum, dawid1999prequential}.

\paragraph{SGD as an estimator for Deep Learning.} Deep Neural Networks (DNN) are typically trained with SGD which does not guarantee convergence to a maximum likelihood solution. Nonetheless, empirically, for ERM, well-tuned SGD finds solutions with good in-distribution generalization. Equivalently, although we cannot guarantee that DNN+SGD achieves a universal code when used as a next-step predictor in prequential MDL, it still gives a valid code length that can be used to tune hyperparameters. Just as different techniques developed for DNN with ERM evaluation, techniques can be developed and compared fairly with prequential MDL. For example, we can compare code length of the different CL techniques or replay strategies to determine their effectiveness. 


\subsection{Individual Sequences: Algorithmic Complexity and Shannon Information Theory}

MDL is also closely related and sometimes phrased in terms of Algorithmic Complexity Theory (ACT) \citep{Hutter:08kolmo,Li:08} instead of Shannon's Information Theory \citep{Shannon:48}. 
With ACT the fundamental concept of {\em information} is defined in terms of symbols and computation, instead of random variables and distributions. 
Quantities such as the entropy of a distribution, the mutual information between random variables and the cross entropy have analogous quantities in ACT: 
Kolmogorov complexity, algorithmic mutual information and description length respectively. 
In ACT however they are defined for individual sequences without the notion of an underlying probabilistic process.
Grünwald and Vitanyi \citep{Grunwald2004-fm} discuss this formally: 
The Kolmogorov complexity for example is a quantity associated with a concrete, individual sequence of symbols. 
If however we consider a stochastic process defining a distribution over such sequences, 
then the expected Kolmogorov complexity is equal to the Entropy of that process (up to an additive constant).
Similarly, the expected description length of sequences with respect to a model corresponds 
to the cross-entropy between an empirical distribution and a model distribution. 
A similar relationship exists for mutual information and algorithmic mutual information.

Minimizing the description length for a given sequence of observations thus corresponds to the ACT analogon of minimizing the cross-entropy given only a single sample from the sequence-generating process.
Much like the cross-entropy is lower-bounded by the entropy of the empirical distribution, 
the description length of a sequence is lower-bounded by its Kolmogorov complexity.






































==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

